Recommender Systems for Online and Mobile Social Networks: A survey

Recommender Systems (RS) currently represent a fundamental tool in online services, especially with the advent of Online Social Networks (OSN). In this case, users generate huge amounts of contents and they can be quickly overloaded by useless information. At the same time, social media represent an important source of information to characterize contents and users' interests. RS can exploit this information to further personalize suggestions and improve the recommendation process. In this paper we present a survey of Recommender Systems designed and implemented for Online and Mobile Social Networks, highlighting how the use of social context information improves the recommendation task, and how standard algorithms must be enhanced and optimized to run in a fully distributed environment, as opportunistic networks. We describe advantages and drawbacks of these systems in terms of algorithms, target domains, evaluation metrics and performance evaluations. Eventually, we present some open research challenges in this area.

==> osn-table.tex <==
\begin{table}[t]
    \centering
    \caption{My caption}
    \label{my-label}
    \begin{tabular}{@{}cccccccll@{}}
        \toprule
        \multicolumn{1}{l}{}               & \multicolumn{6}{c}{\textbf{RS Method}}                                                                                                                                                                         & \multicolumn{2}{c}{\textbf{Evaluation}}                                                                                                                        \\ \midrule
        \multicolumn{1}{|c|}{\textbf{Ref}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{CB}} & \multicolumn{1}{c|}{\textbf{MF}} & \multicolumn{1}{c|}{\textbf{TF}} & \multicolumn{1}{c|}{\textbf{G}} & \multicolumn{1}{c|}{\textbf{DL}} & \multicolumn{1}{c|}{\textbf{Datasets}}                                          & \multicolumn{1}{c|}{\textbf{Metrics}}                                        \\ \midrule
        \cite{ma2008sorec}                 &                                  &                                  & \checkmark                       &                                  &                                 &                                  & - Epinions                                                                      & - MAE                                                                        \\
        \cite{jamali2010matrix}            &                                  &                                  & \checkmark                       &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Flixster\\ - Epinions\end{tabular}                 & - RMSE                                                                       \\
        \cite{ma2011recommender}           &                                  &                                  & \checkmark                       &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Douban\\ - Epinions\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}- MAE\\ - RMSE\end{tabular}                       \\
        \cite{ma2009learning}              &                                  &                                  & \checkmark                       &                                  &                                 &                                  & - Epinions                                                                      & \begin{tabular}[c]{@{}l@{}}- MAE\\ - RMSE\end{tabular}                       \\
        \cite{sun2015recommender}          &                                  &                                  & \checkmark                       &                                  &                                 &                                  & - Delicious                                                                     & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{reafee2016power}             &                                  &                                  & \checkmark                       &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Last.fm\\ - Douban\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}- MAE\\ - RMSE\end{tabular}                       \\
        \cite{kim2014framework}            & \checkmark                       & \checkmark                       &                                  &                                  &                                 &                                  & - MovieLens                                                                     & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\\ - F-measure\end{tabular} \\
        \cite{sigurbjornsson2008flickr}    &                                  & \checkmark                       &                                  &                                  &                                 &                                  & - Flickr                                                                        & \begin{tabular}[c]{@{}l@{}}- MRR\\ - Precision\\ - Recall\end{tabular}       \\
        \cite{firan2007benefit}            & \checkmark                       &                                  &                                  &                                  &                                 &                                  & - Last.fm                                                                       & \begin{tabular}[c]{@{}l@{}}- nDCG\\ - Novelty\end{tabular}                   \\
        \cite{peng2010collaborative}       & \checkmark                       &                                  &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Delicious\\ - CiteULike\\ - Bibsonomy\end{tabular} & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\\ - F-measure\end{tabular} \\
        \cite{shepitsen2008personalized}   &                                  & \checkmark                       &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Delicious\\ - Last.fm\end{tabular}                 & Custom                                                                       \\
        \cite{liang2010connecting}         & \checkmark                       &                                  &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Amazon\\ - CiteULike\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{symeonidis2008tag}           &                                  &                                  &                                  & \checkmark                       &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Last.fm\\ - Bibsonomy\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{rendle2009learning}          &                                  &                                  &                                  & \checkmark                       &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Last.fm\\ - Bibsonomy\end{tabular}                 & - F-measure                                                                  \\
        \cite{zhang2010personalized}       &                                  &                                  &                                  &                                  & \checkmark                      &                                  & \begin{tabular}[c]{@{}l@{}}- Delicious\\ - Movielens\\ - Bibsonomy\end{tabular} & \begin{tabular}[c]{@{}l@{}}- AUC\\ - Recall\\ - Novelty\end{tabular}         \\
        \cite{arnaboldi2016pliers}         &                                  &                                  &                                  &                                  & \checkmark                      &                                  & \begin{tabular}[c]{@{}l@{}}- Movielens\\ - Delicious\\ - Twitter\end{tabular}   & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\\ - Novelty\end{tabular}   \\
        \cite{zuo2016tag}                  &                                  &                                  &                                  &                                  &                                 & \checkmark                       & \begin{tabular}[c]{@{}l@{}}- Last.fm\\ - Delicious\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{ijcai2017-446}               &                                  &                                  &                                  &                                  &                                 & \checkmark                       & \begin{tabular}[c]{@{}l@{}}- Delicious\\ - Last.fm\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\\ - F1-score\end{tabular}  \\
        \cite{shi2011personalized}         &                                  &                                  & \checkmark                       &                                  &                                 &                                  & - Flickr                                                                        & - MAP                                                                        \\
        \cite{levi2012finding}             &                                  & \checkmark                       &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Tripadvisor\\ - Venere\end{tabular}                & Custom                                                                       \\
        \cite{yang2013fine}                &                                  &                                  &                                  & \checkmark                       &                                 &                                  & - Foursquare                                                                    & \begin{tabular}[c]{@{}l@{}}- MAP\\ - MAS\end{tabular}                        \\
        \cite{wang2017location}            &                                  & \checkmark                       &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Yelp\\ - Foursquare\end{tabular}                   & - Precision                                                                  \\
        \cite{yin2016adapting}             &                                  & \checkmark                       &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Yelp\\ - Foursquare\end{tabular}                   & Custom                                                                       \\
        \cite{ye2010location}              & \checkmark                       &                                  &                                  &                                  &                                 &                                  & - Foursquare                                                                    & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{ye2011exploiting}            & \checkmark                       &                                  &                                  &                                  &                                 &                                  & \begin{tabular}[c]{@{}l@{}}- Foursquare\\ - Whrll\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{zheng2009mining}             &                                  &                                  &                                  &                                  & \checkmark                      &                                  & Custom                                                                          & - Map                                                                        \\
        \cite{scellato2011exploiting}      &                                  & \checkmark                       &                                  &                                  &                                 &                                  & - Gowalla                                                                       & - ROC curve                                                                  \\
        \cite{yu2011geo}                   &                                  &                                  &                                  &                                  & \checkmark                      &                                  & \begin{tabular}[c]{@{}l@{}}- syntetic\\ - MIT\end{tabular}                      & - Precision                                                                  \\
        \cite{xiao2010finding}             &                                  & \checkmark                       &                                  &                                  &                                 &                                  & Custom                                                                          & - nDCG                                                                       \\
        \cite{zheng2010collaborative}      &                                  &                                  &                                  & \checkmark                       &                                 &                                  & Custom                                                                          & - nDCG                                                                       \\
        \cite{symeonidis2011geo}           &                                  &                                  &                                  & \checkmark                       & \checkmark                      &                                  & Custom                                                                          & \begin{tabular}[c]{@{}l@{}}- Precision\\ - Recall\end{tabular}               \\
        \cite{zheng2012towards}            & \checkmark                       &                                  & \checkmark                       & \checkmark                       &                                 &                                  & Custom                                                                          & \begin{tabular}[c]{@{}l@{}}- AUC\\ - RMSE\end{tabular}                       \\
        \cite{palovics2017location}        &                                  & \checkmark                       & \checkmark                       &                                  &                                 &                                  & - Twitter                                                                       & - DCG                                                                        \\ \bottomrule
    \end{tabular}
\end{table}
